Snowmass2021 Cosmic Frontier White Paper: Calibrations and backgrounds for dark matter direct detection

Future dark matter direct detection experiments will reach unprecedented levels of sensitivity. Achieving this sensitivity will require more precise models of signal and background rates in future detectors. Improving the precision of signal and background modeling goes hand-in-hand with novel calibration techniques that can probe rare processes and lower threshold detector response. The goal of this white paper is to outline community needs to meet the background and calibration requirements of next-generation dark matter direct detection experiments.

==> Sections/2.3-Coherent_excitations.tex <==
\subsection{Coherent-Excitation Calibration \small{(\emph{Lead: Scott Hertel})}}
\label{ssec:coherent}


==> Sections/3.4-Inactive_materials_beta-gamma.tex <==
\subsection{Betas \& Gammas from Inactive Materials}
\label{ssec:inactive_materials}

(e.g. U, Th, Pb210, K40)

